Compilation of Coordinated Choice

Recently, we have proposed coordinated choices, which are nondeterministic choices equipped with names. The main characteristic of coordinated choices is that they synchronize nondeterministic decision among choices of the same name. The motivation of the synchronization mechanism is to solve a theoretical problem. So, as a practical programming language, we still want to use coordinated choices like standard ones. In other words, we want to avoid synchronization. Now, there are two problems: (i) practically, it is a bit complicated work to write a program using coordinated choices in which execution synchronization never happens; and (ii) theoretically, it is unknown whether any programs using standard choices can be written by using only coordinated ones. In this paper, we define two simply typed lambda calculi called $\lambda^\parallel$ equipped with standard choices and $\lambda^{\parallel\omega}$ equipped with coordinated choices, and give compilation rules from the former into the latter. The challenge is to show the correctness of the compilation because behavioral correspondence between expressions before and after compiling cannot be defined directly by the compilation rules. For the challenge, we give an effect system for $\lambda^{\parallel\omega}$ that characterizes expressions in which execution synchronization never happens. Then, we show that all compiled expressions can be typed by the effect system. As a result, we can easily show the correctness because the main concern of the correctness is whether synchronization happens or not.

==> figures/seval.tex <==
  \begin{rules}[prefix=SE]
    \infax[Abs]{
      \(\texttt{\textcolor{red}{<<no parses (char 9): \mbox{$\backslash{}$}x.e // \mbox{$\backslash{}$}***x.e >>}}\)
    }
    \infte[App]{
      \(\texttt{\textcolor{red}{<<no parses (char 7): e1 // \mbox{$\backslash{}$}***x.e1' >>}}\)
    }{
      \(\texttt{\textcolor{red}{<<no parses (char 7): e2 // v*** >>}}\)
    }{
      \(\texttt{\textcolor{red}{<<no parses (char 14): e1'.\{v/x\} // r*** >>}}\)
    }{
      \(\texttt{\textcolor{red}{<<no parses (char 10): e1 e2 // r*** >>}}\)
    }
    \infbi[Choice]{
      \(\texttt{\textcolor{red}{<<no parses (char 7): e1 // r***1 >>}}\)
    }{
      \(\texttt{\textcolor{red}{<<no parses (char 7): e2 // r***2 >>}}\)
    }{
      \(\texttt{\textcolor{red}{<<no parses (char 15): (e1 \mbox{$\mid$}\mbox{$\mid$} e2) // (***r1 \mbox{$\mid$}\mbox{$\mid$} r2) >>}}\)
    }
    \infbi[AppDistL]{
      \(\texttt{\textcolor{red}{<<no parses (char 7): e1 // (***r11 \mbox{$\mid$}\mbox{$\mid$} r12) >>}}\)
    }{
      \(\texttt{\textcolor{red}{<<no parses (char 3): (r1***1 e2 \mbox{$\mid$}\mbox{$\mid$} r12 e2) // r >>}}\)
    }{
      \(\texttt{\textcolor{red}{<<no parses (char 10): e1 e2 // r*** >>}}\)
    }
    \infte[AppDistR]{
      \(\texttt{\textcolor{red}{<<no parses (char 7): e1 // v***1 >>}}\)
    }{
      \(\texttt{\textcolor{red}{<<no parses (char 7): e2 // (***r21 \mbox{$\mid$}\mbox{$\mid$} r22) >>}}\)
    }{
      \(\texttt{\textcolor{red}{<<no parses (char 5): (v1 r***21 \mbox{$\mid$}\mbox{$\mid$} v1 r22) // r >>}}\)
    }{
      \(\texttt{\textcolor{red}{<<no parses (char 10): e1 e2 // r*** >>}}\)
    }
  \end{rules}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../note.otex"
%%% End:


==> figures/tssemantics.tex <==
\begin{rules}
  \infax[BetaSigma]{
    \(\texttt{\textcolor{red}{<<no parses (char 14): (\mbox{$\backslash{}$}x.\mbox{$\backslash{}$}'a.M) V p*** ===>D M.\{V/x\}.\{p/'a\} >>}}\)
  }
  \infun[AppL]{
    \(\texttt{\textcolor{red}{<<no parses (char 10): M ===>D M'*** >>}}\)
  }{
    \(\texttt{\textcolor{red}{<<no parses (char 3): M N*** p ===>D M' N p >>}}\)
  }
  \infun[AppR]{
    \(\texttt{\textcolor{red}{<<no parses (char 1): N*** ===>D N' >>}}\)
  }{
    \(\texttt{\textcolor{red}{<<no parses (char 3): V N*** p ===>D V N' p >>}}\)
  }
  \infun[ChoiceL]{
    \(\texttt{\textcolor{red}{<<no parses (char 9): M ===>D\mbox{$\backslash{}$}/***\{p+\} M' >>}}\)
  }{
    \(\texttt{\textcolor{red}{<<no parses (char 6): (M \mbox{$\mid$}\mbox{$\mid$}p*** N) ===>D (M' \mbox{$\mid$}\mbox{$\mid$}p N) >>}}\)
  }
  \infun[ChoiceR]{
    \(\texttt{\textcolor{red}{<<no parses (char 1): N*** ===>D\mbox{$\backslash{}$}/\{p-\} N' >>}}\)
  }{
    \(\texttt{\textcolor{red}{<<no parses (char 6): (M \mbox{$\mid$}\mbox{$\mid$}p*** N) ===>D (M \mbox{$\mid$}\mbox{$\mid$}p N') >>}}\)
  }
  \infax[DistAppL]{
    \(\texttt{\textcolor{red}{<<no parses (char 6): (M \mbox{$\mid$}\mbox{$\mid$}p*** N) L q ===>D (M L q \mbox{$\mid$}\mbox{$\mid$}p N L q) >>}}\)
  }
  \infax[DistAppR]{
    \(\texttt{\textcolor{red}{<<no parses (char 8): V (M \mbox{$\mid$}\mbox{$\mid$}p*** N) q ===>D (V M q \mbox{$\mid$}\mbox{$\mid$}p V N q) >>}}\)
  }
\end{rules}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../note.otex"
%%% End:

